One Training for Multiple Deployments: Polar-based Adaptive BEV Perception for Autonomous Driving

Current on-board chips usually have different computing power, which means multiple training processes are needed for adapting the same learning-based algorithm to different chips, costing huge computing resources. The situation becomes even worse for 3D perception methods with large models. Previous vision-centric 3D perception approaches are trained with regular grid-represented feature maps of fixed resolutions, which is not applicable to adapt to other grid scales, limiting wider deployment. In this paper, we leverage the Polar representation when constructing the BEV feature map from images in order to achieve the goal of training once for multiple deployments. Specifically, the feature along rays in Polar space can be easily adaptively sampled and projected to the feature in Cartesian space with arbitrary resolutions. To further improve the adaptation capability, we make multi-scale contextual information interact with each other to enhance the feature representation. Experiments on a large-scale autonomous driving dataset show that our method outperforms others as for the good property of one training for multiple deployments.

==> sections/backup.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}
% 背景：真实世界的3D物体的size大小范围很大，从长度10m+的车到半径20cm的锥桶，它们的识别需要不同尺度的BEV特征，这个是很难在一个单一尺度的feature map上被包含的
% 抛出一个问题：目前SoTA的三维检测器通常是用多个尺度的检测器聚合而来的，但是实际使用中我们无法在车端同时部署多个尺度检测器；基于Transformer范式的BEV感知网络，拟合较慢，显存开销较大，不利于部署，对于多尺度感知场景更加不友好
% 我们的方法：基于Polar的感知范式更符合环视BEV的视场分布特性，而Transformer是将笛卡尔坐标映射到Polar坐标系的有效手段。使用多分支的三维检测器可以在不同尺度的场景中获得均衡的性能，使用统一的主干网络，利用较少的网络参数。


\end{abstract}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{INTRODUCTION}
% 一. 1.解决的问题：BEV感知是自动驾驶领域的重要问题，，单尺度BEV特征无法更好的适应实际应用场景中不同大小的目标。
%     2.问题的重要性：多场景(尺度)BEV特征的部署更有利于检测场景中不同的目标(eg. 卡车，自行车，行人)
    


\begin{itemize}
\item Single network for multi-scale detection.
\item Deformable-Multi-scale feature alignment


\end{itemize}


\section{RELATED WORK}

\subsection{Selecting a Template (Heading 2)}



\subsection{Homograph-based PV2BEV}
\subsection{MLP based PV2BEV}
\subsection{Transformer based PV2BEV}

\begin{figure*}
    \centering
%	\begin{minipage}[t]{0.92\linewidth}
	\includegraphics[width=1.0\textwidth]{Figures/Network.png} 
%	\end{minipage}
\caption{network architecture.}
\vspace{-2ex}
\label{fig:network}
\end{figure*}


\section{Multi-Scale BEV Perception Network}
We propose a novel Polar-based 3D object detection paradigm in Bird-Eye-View (BEV). It takes multi-view RGB images with corresponding projection matrices (including intrinsic and extrinsic parameters) as input, and the outputs are the 3D bounding box parameters of the objects. The surround-view images ${X^{H \times W \times 3}}$ are encoded by a single shared backbone following [BEVerse] to obtain multi-scale 2D representations ${F_l}\} _l^{{N_{scale}}}$ with shape ${\frac{H}{{{2}^{i+1}}}\times \frac{W}{{{2}^{i+1}}}\times C}$, and unify the spatial resolution of 2D features with shape ${{{X}_{1}}^{\frac{H}{16}\times \frac{W}{16}\times C}}$ by FPNLSS[BEVDet]. The Column-wise encoder projects the image columns in Cartesian coordinate to the Polar rays in Cylindrical coordinate,Polar map describes the BEV Perception space more concretely. Further, a Multi-scale interaction encoder helps correlate various-scale objects contextual representations across all feature levels. Finally, a Multi-scale alignment module aligns the transformation offsets of diversely scaled BEV grids. The details of the overall architecture are described as Fig *.
\subsection{Column-wise transformer module}
For the BEV detection task, one of key challenges is the transformation between the 2D images and the BEV space. Many recent studies[LSS,BEVerse,petr] establish camera frustum ${{c}_{i}}={{({{u}_{i}}\times {{d}_{i}},{{v}_{i}}\times{{d}_{i}},{{d}_{i}},1)}^{T}}$, where ${({{u}_{i}},{{v}_{i}}}$ is the pixel,${{{d}_{i}}}$ is radial distance, with explicit depth prediction in the image coordinate, and transform the points to the 3D space with camera’s parameters, then performs a cumulative sum and subtracts process to the depth bins obtaining the BEV features. Such an implementation can bring the projection error, since the depth prediction process is difficulty. [BEDepth] apply the ground-truth depth from Lidar to make explicit depth supervision, it exactly enhances the network performance. However, for the vision-center BEV task, the Lidar signals are superfluous, and brings a large amount of computations. The Polar-based paradigm is more suitable for the surround-view perception and our Column-polar wise transform module boosts the image-to-BEV view transformation without ill-posed depth estimation, aligning the pixel coordinate and polar coordinate. First, we constract the camera frustum without dense meshgrid along depth axis, unlike [polarformer,polardetr] the relationship of image columns and polar rays only relies on the farside points relative to cameras, so the azimuth ${{\sigma }_{i}}$ can be calculate as: ${{\sigma }_{i}}=\arctan (\frac{{{y}^{w}}}{{{x}^{w}}})$ ,where i is the index of image columns. And the Polar distance range is decided by iamge shape: ${{d}_{i}}=\sqrt{{{(\frac{H}{2})}^{2}}+{{(\frac{W}{2})}^{2}}}$. For each Polar ray query, the congruent relationships are built by our Column-wise cross-attention(CCA) as shown in Fig. *. Benefiting from the exact estimation of the ${{\sigma }_{i}}$, our CCA can focus more on the view overlapping regions, We enumerate columns projected to the same ray and adaptively assign higher attention weights. In order to facilitate the deployment of different computing power platforms, our network can adapt to various granularities of Cartesian BEV grids distribution. 

\subsection{Multi-scale alignment module}
To make our algorithm adapt to various BEV ranges and try to explore balance performance for different object scales. We exploit multi-scale BEV interaction encoder to interact with different granularity of contextual information from sampled Cartesian BEV maps, our multi-scale BEV interaction encoder is expressed as:
\begin{equation}
\begin{aligned}
    &MSBEVDeformAttn({{b}_{q}},\overset{\wedge }{\mathop{{{r}_{q}}}}\,,\{{{b}^{s}}\}_{s=1}^{S})= \\ &\sum\limits_{h}^{H}{{{W}_{h}}[\sum\limits_{s=1}^{S}{\sum\limits_{r=1}^{R}{{{A}_{hsqr}}{{W}_{h}}^{'}}}{{b}^{s}}({{\sigma }_{s}}(\overset{\wedge }{\mathop{{{r}_{q}}}}\,)+\Delta {{f}_{hsqr}})]}
\end{aligned}
\end{equation}
Where ${{b}_{q}}$ is the BEV query feature, $\overset{\Lambda }{\mathop{{{r}_{q}}}}\,\in {{[0,1]}^{2}}$ represent the reference points normalized coordinates for scale formulation. ${{b}^{s}}$ is the multi-scale BEV features, 


%project image features from perspective view to BEV 
%A. polar self-attention
% B. adaptivity overlap-region attention

\subsection{Column-wise encoder}
% A. Multi-scale feature interaction
% B. Multi-scale feature aggregation
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[t]
  \centering
  \caption{Ablation Study}
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
    \toprule
    Methods & Resolution & mAP   & mATE  & mASE  & mAOE  & mAVE  & mAAE  & NDS \\
    \midrule
    BEVDet & 704×256 & 29.4  & 0.686 & 0.278 & 0.547 & 0.865 & 0.261 & 0.384 \\
    \midrule
    Polar-wise module  & 704×256 & 30.29 & 0.6956 & 0.2768 & 0.5486 & 0.8978 & 0.2425 & 0.3853 \\
    \midrule
    Multiscale alignment & 704×256 &       &       &       &       &       &       &  \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%

\begin{table*}[htbp]
  \centering
  \caption{Comparison of Multi-scale BEV Resolution}
  \scalebox{0.8}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
    \toprule
    Module & Output size & Training Head & NDS   & mAP   & mATE  & mASE  & mAOE  & mAVE  & mAAE \\
    \midrule
    \multirow{3}[2]{*}{FaPN\_128} & 128×128 & \multirow{3}[2]{*}{128 head} & 0.3769 & 0.3047 & 0.7234 & 0.275 & 0.527 & 0.9866 & 0.2428 \\
          & 200×200 &       & 0.3549 & 0.283 & 0.7798 & 0.293 & 0.5414 & 1.0251 & 0.2518 \\
          & 256×256 &       & 0.3304 & 0.2489 & 0.8427 & 0.309 & 0.5778 & 0.9715 & 0.2392 \\
    \midrule
    \multirow{3}[2]{*}{FaPN\_200} & 128×128 & \multirow{3}[2]{*}{200 head} & 0.3421 & 0.2138 & 0.818 & 0.2897 & 0.5627 & 0.7586 & 0.2191 \\
          & 200×200 &       & 0.3859 & 0.3046 & 0.7124 & 0.2715 & 0.5175 & 0.9161 & 0.2468 \\
          & 256×256 &       & 0.3746 & 0.2927 & 0.7229 & 0.2825 & 0.5337 & 0.9363 & 0.242 \\
    \midrule
    \multirow{3}[2]{*}{Interpolation} & 128×128 & \multirow{3}[2]{*}{200 head} & 0.3488 & 0.2444 & 0.8037 & 0.2893 & 0.5302 & 0.848 & 0.2627 \\
          & 200×200 &       & 0.3846 & 0.3083 & 0.6922 & 0.2743 & 0.5001 & 0.9594 & 0.2692 \\
          & 256×256 &       & 0.3748 & 0.2993 & 0.6891 & 0.282 & 0.5033 & 1.0012 & 0.2739 \\
    \midrule
    \multirow{3}[2]{*}{BEVDet} & 128×128 & \multirow{3}[2]{*}{128 head} & 0.4037 & 0.308 & 0.6648 & 0.2729 & 0.5323 & 0.8277 & 0.205 \\
          & 200×200 &       & 0.3903 & 0.2977 & 0.6865 & 0.2826 & 0.538 & 0.8772 & 0.2016 \\
          & 256×256 &       & 0.2755 & 0.2015 & 1.0046 & 0.3289 & 0.7024 & 1.0103 & 0.2214 \\
    \bottomrule
    \end{tabular}}%
  \label{tab:addlabel}%
\end{table*}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{ Comparison of recent works on the nuScenes val set.}
    \begin{tabular}{c|c|r|r|r|r|r|r|r}
    \toprule
    Methods & Image Size & \multicolumn{1}{c|}{NDS} & \multicolumn{1}{c|}{mAP} & \multicolumn{1}{c|}{mATE} & \multicolumn{1}{c|}{mASE} & \multicolumn{1}{c|}{mAOE} & \multicolumn{1}{c|}{mAVE} & \multicolumn{1}{c}{mAAE} \\
    \midrule
    CenterNet &  -    & \multicolumn{1}{c|}{0.328} & \multicolumn{1}{c|}{0.306} & \multicolumn{1}{c|}{0.716} & \multicolumn{1}{c|}{0.264} & \multicolumn{1}{c|}{0.609} & \multicolumn{1}{c|}{1.426} & \multicolumn{1}{c}{0.658} \\
    FCOS3D & 1600×900 & \multicolumn{1}{c|}{0.372} & \multicolumn{1}{c|}{0.295} & \multicolumn{1}{c|}{0.806} & \multicolumn{1}{c|}{0.268} & \multicolumn{1}{c|}{0.511} & \multicolumn{1}{c|}{1.315} & \multicolumn{1}{c}{0.17} \\
    DETR3D & 1600×900 & \multicolumn{1}{c|}{0.374} & \multicolumn{1}{c|}{0.303} & \multicolumn{1}{c|}{0.86} & \multicolumn{1}{c|}{0.278} & \multicolumn{1}{c|}{0.437} & \multicolumn{1}{c|}{0.967} & \multicolumn{1}{c}{0.235} \\
    PGD   & 1600×900 & \multicolumn{1}{c|}{0.409} & \multicolumn{1}{c|}{0.335} & \multicolumn{1}{c|}{0.732} & \multicolumn{1}{c|}{0.263} & \multicolumn{1}{c|}{0.423} & \multicolumn{1}{c|}{1.285} & \multicolumn{1}{c}{0.172} \\
    PETR  & 1056×384 & \multicolumn{1}{c|}{0.381} & \multicolumn{1}{c|}{0.313} & \multicolumn{1}{c|}{0.768} & \multicolumn{1}{c|}{0.278} & \multicolumn{1}{c|}{0.564} & \multicolumn{1}{c|}{0.923} & \multicolumn{1}{c}{0.225} \\
    BEVDet & 704×256 & \multicolumn{1}{c|}{0.379} & \multicolumn{1}{c|}{0.298} & \multicolumn{1}{c|}{0.725} & \multicolumn{1}{c|}{0.279} & \multicolumn{1}{c|}{0.589} & \multicolumn{1}{c|}{0.86} & \multicolumn{1}{c}{0.245} \\
    PersDet & 704×256 & \multicolumn{1}{c|}{0.389} & \multicolumn{1}{c|}{0.319} & \multicolumn{1}{c|}{0.676} & \multicolumn{1}{c|}{0.284} & \multicolumn{1}{c|}{0.589} & \multicolumn{1}{c|}{0.924} & \multicolumn{1}{c}{0.229} \\
    CaDNN & 704×256 & \multicolumn{1}{c|}{0.37} & \multicolumn{1}{c|}{0.294} & \multicolumn{1}{c|}{0.702} & \multicolumn{1}{c|}{0.283} & \multicolumn{1}{c|}{0.579} & \multicolumn{1}{c|}{0.988} & \multicolumn{1}{c}{0.222} \\
    ours  & 704×256 &       &       &       &       &       &       &  \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


% Table generated by Excel2LaTeX from sheet 'Sheet1'




\section{Experiment}

\subsection{Qualitative evaluation}

%nuscences val:网络最好的结果与其他方法对比； FCOS3D pretrained; CBGS;
% 1.先训出最好的结果，然后上FCOS3D(val); DD3D(test)


%nuscences test:DD3D pretrained

\subsection{Network generalization performance}
%A. 网络泛化性能ablation study(128.200.256)
%多场景，多尺度部署性能
%B. 与其他网络泛化性能对比




\subsection{Ablation study}
%不同module的性能
% Table generated by Excel2LaTeX from sheet 'Sheet1'


\subsection{Efficiency evaluation}
% 与Transformer方法的运行效率对比
%性能差异较大还需要比吗？



\section{CONCLUSIONS}

% A conclusion section is not required. Although a conclusion may review the main points of the paper, do not replicate the abstract as the conclusion. A conclusion might elaborate on the importance of the work or suggest applications and extensions. 

\addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
                                  % on the last page of the document manually. It shortens
                                  % the textheight of the last page by a suitable amount.
                                  % This command does not take effect until the next page
                                  % so it should come on the page before the last. Make
                                  % sure that you do not shorten the textheight too much.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{APPENDIX}

% Appendixes should appear before the acknowledgment.

\section*{ACKNOWLEDGMENT}

% The preferred spelling of the word ÒacknowledgmentÓ in America is without an ÒeÓ after the ÒgÓ. Avoid the stilted expression, ÒOne of us (R. B. G.) thanks . . .Ó  Instead, try ÒR. B. G. thanksÓ. Put sponsor acknowledgments in the unnumbered footnote on the first page.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.



%\begin{thebibliography}{99}

% \bibitem{c1} G. O. Young, ÒSynthetic structure of industrial plastics (Book style with paper title and editor),Ó 	in Plastics, 2nd ed. vol. 3, J. Peters, Ed.  New York: McGraw-Hill, 1964, pp. 15Ð64.
% \bibitem{c2} W.-K. Chen, Linear Networks and Systems (Book style).	Belmont, CA: Wadsworth, 1993, pp. 123Ð135.
% \bibitem{c3} H. Poor, An Introduction to Signal Detection and Estimation.   New York: Springer-Verlag, 1985, ch. 4.
% \bibitem{c4} B. Smith, ÒAn approach to graphs of linear forms (Unpublished work style),Ó unpublished.
% \bibitem{c5} E. H. Miller, ÒA note on reflector arrays (Periodical styleÑAccepted for publication),Ó IEEE Trans. Antennas Propagat., to be publised.
% \bibitem{c6} J. Wang, ÒFundamentals of erbium-doped fiber amplifiers arrays (Periodical styleÑSubmitted for publication),Ó IEEE J. Quantum Electron., submitted for publication.
% \bibitem{c7} C. J. Kaufman, Rocky Mountain Research Lab., Boulder, CO, private communication, May 1995.
% \bibitem{c8} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ÒElectron spectroscopy studies on magneto-optical media and plastic substrate interfaces(Translation Journals style),Ó IEEE Transl. J. Magn.Jpn., vol. 2, Aug. 1987, pp. 740Ð741 [Dig. 9th Annu. Conf. Magnetics Japan, 1982, p. 301].
% \bibitem{c9} M. Young, The Techincal Writers Handbook.  Mill Valley, CA: University Science, 1989.
% \bibitem{c10} J. U. Duncombe, ÒInfrared navigationÑPart I: An assessment of feasibility (Periodical style),Ó IEEE Trans. Electron Devices, vol. ED-11, pp. 34Ð39, Jan. 1959.
% \bibitem{c11} S. Chen, B. Mulgrew, and P. M. Grant, ÒA clustering technique for digital communications channel equalization using radial basis function networks,Ó IEEE Trans. Neural Networks, vol. 4, pp. 570Ð578, July 1993.
% \bibitem{c12} R. W. Lucky, ÒAutomatic equalization for digital communication,Ó Bell Syst. Tech. J., vol. 44, no. 4, pp. 547Ð588, Apr. 1965.
% \bibitem{c13} S. P. Bingulac, ÒOn the compatibility of adaptive controllers (Published Conference Proceedings style),Ó in Proc. 4th Annu. Allerton Conf. Circuits and Systems Theory, New York, 1994, pp. 8Ð16.
% \bibitem{c14} G. R. Faulhaber, ÒDesign of service systems with priority reservation,Ó in Conf. Rec. 1995 IEEE Int. Conf. Communications, pp. 3Ð8.
% \bibitem{c15} W. D. Doyle, ÒMagnetization reversal in films with biaxial anisotropy,Ó in 1987 Proc. INTERMAG Conf., pp. 2.2-1Ð2.2-6.
% \bibitem{c16} G. W. Juette and L. E. Zeffanella, ÒRadio noise currents n short sections on bundle conductors (Presented Conference Paper style),Ó presented at the IEEE Summer power Meeting, Dallas, TX, June 22Ð27, 1990, Paper 90 SM 690-0 PWRS.
% \bibitem{c17} J. G. Kreifeldt, ÒAn analysis of surface-detected EMG as an amplitude-modulated noise,Ó presented at the 1989 Int. Conf. Medicine and Biological Engineering, Chicago, IL.
% \bibitem{c18} J. Williams, ÒNarrow-band analyzer (Thesis or Dissertation style),Ó Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, 1993. 
% \bibitem{c19} N. Kawasaki, ÒParametric study of thermal and chemical nonequilibrium nozzle flow,Ó M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.
% \bibitem{c20} J. P. Wilkinson, ÒNonlinear resonant circuit devices (Patent style),Ó U.S. Patent 3 624 12, July 16, 1990. 



